Sentence-Level BERT and Multi-Task Learning of Age and Gender in Social Media

Social media currently provide a window on our lives, making it possible to learn how people from different places, with different backgrounds, ages, and genders use language. In this work we exploit a newly-created Arabic dataset with ground truth age and gender labels to learn these attributes both individually and in a multi-task setting at the sentence level. Our models are based on variations of deep bidirectional neural networks. More specifically, we build models with gated recurrent units and bidirectional encoder representations from transformers (BERT). We show the utility of multi-task learning (MTL) on the two tasks and identify task-specific attention as a superior choice in this context. We also find that a single-task BERT model outperform our best MTL models on the two tasks. We report tweet-level accuracy of 51.43% for the age task (three-way) and 65.30% on the gender task (binary), both of which outperforms our baselines with a large margin. Our models are language-agnostic, and so can be applied to other languages.

==> bert.tex <==

\subsection{BERT}\label{subsec:bert}
%-----------------
BERT~\cite{devlin2018bert} stands for \textbf{B}idirectional \textbf{E}ncoder \textbf{R}epresentations from \textbf{T}ransformers. It is an approach for pre-training language representations that involves two unsupervised learning tasks, (1) \textit{masked language models (Masked LM)} and (2) \textit{next sentence prediction}. Since BERT uses bidirectional conditioning, a given percentage of random input tokens are masked and the model attempts to predict these masked tokens. %This is the Masked LM task, where masked tokens are simply replaced by a string \texttt{[MASK]} 
.~\citet{devlin2018bert} mask 15\% of the tokens (the authors use \textit{word pieces}) and feed the final hidden vectors of these masked tokens to an output softmax over the vocabulary. The next sentence prediction task of BERT is also straightforward.~\citet{devlin2018bert} simply cast the task as binary classification. For a given sentence \texttt{S}, two sentences \texttt{A} and \texttt{B} are generated where \texttt{A} (positive class) is an actual sentence from the corpus and \texttt{B} is a randomly chosen sentence (negative class). Once trained on an unlabeled dataset, BERT can then be fine-tuned with supervised data.

==> bert_analysis.tex <==
\section{BERT Model Analysis}\label{sec:seq-length}
%------------------------------------------
%--------


%\begin{landscape}
\begin{table}[]
\centering
%\resizebox{\textwidth}{!}{%
\begin{tabular}{l|cc} \hline 
\textbf{Setting} & \textbf{Age} & \textbf{Gender} \\ \hline 
\textbf{maj-base} & 35.53 & 53.47 \\
\textbf{small-GRU} & 36.13 & 53.39 \\ \hline
\textbf{all-lengths} & 51.44 & 65.31 \\ \hline 
\textbf{1-5 tokens} & 49.96 & 63.64 \\
\textbf{6-10 tokens} & 52.86 & 65.97 \\
\textbf{11-15 tokens} & 51.94 & 66.76 \\
\textbf{15-20 tokens} & 52.37 & 66.95 \\
\textbf{21-25 tokens} & 51.99 & 66.54 \\
\textbf{25-30 tokens} & 51.76 & 66.11 \\
 \hline 
\end{tabular}%
%}
\caption{BERT performance in accuracy on TEST data per sequence length (in tokens).}
\label{tab:res_bert_length}
\end{table}
%\end{landscape}
%-------------

The Transformer architecture on which BERT is based is intended to allow the model to keep information it sees at early stages in the sequence and hence should be able to handle longer sequences better than other recurrence- and convolution-based nets. We perform an analysis based on the sequence length of TEST examples, to identify how BERT could be performing differently on tweets of different lengths. We note that Twitter posts are usually short (i.e., a maximum of 280 characters, up from their historical cut-off point of 140 characters). As Table~\ref{tab:res_bert_length} shows, for the two tasks, BERT performs better on sequences of at least 6 tokens than shorter sequences. We also note that results on the longest sequences (e.g., more than 21 tokens), while better than those on very short tweets, are not necessarily the best. We suspect that a percentage of the longer tweets (i.e., $>$ 21 words) might be automatically generated by APIs (such as APIs that automatically post religious or literary content on behalf of users) or tackle topics that do not vary observably across the age and gender divide. In the future, we intend to further analyze model performance, including with respect to its utility on sequences of varying length.


==> mtl.tex <==
%-----------------------------
\subsection{Multi-Task Learning}
\begin{figure}[h]
\centering
\frame{\includegraphics[width=0.4\textwidth]{images/mtl_1}}
\caption{Our MTL network for city, state, and country. The three tasks share 2 hidden layers, with each task having its independent attention layer.}
\label{fig:mtl_t_spec_attn}
\end{figure}
%-----------------
We investigate the utility of \textit{multi-task learning} (MTL) for language ID. The intuition behind MTL is that many real-world tasks involve making predictions about closely related labels or outcomes. For related tasks, MTL helps achieve inductive transfer between the various tasks by leveraging additional sources of information from some of the tasks to improve performance on the target task~\cite{caruana1993}. By using training signals for related tasks, MTL allows a learner to prefer hypotheses that explain more than one task~\cite{caruana1997multitask} and also helps regularize models.

In single task learning, an independent network is trained in isolation for each task.
In contrast, in MTL, a number of tasks are learned together in a single network, with each task having its own output. An MTL network has a shared input, and one or more hidden layers that are shared between all the tasks. Backpropagation is then applied in parallel on all outputs. In our case, we train a single network for our city, state, and country tasks with one output for each of the three tasks. Figure ~\ref{fig:mtl_t_spec_attn} is an illustration of an MTL network for our 3 tasks, with 2 shared hidden BiGRU layers and a task-specific (i.e., independent) BiGRU attention layer. In our current work, each of the three tasks has its own loss function, with the MTL loss computed as:

%-----------------
\begin{equation}
\begin{multlined}
 \mathcal{L}(\theta_{MTL})&= \left(\mathcal{L}(\theta_{city}) + \mathcal{L}(\theta_{state})+\mathcal{L}(\theta_{country}) \right) / 3 \\ 
 \end{multlined}
\end{equation}

We now introduce the Transformer~\cite{vaswani2017attention}, since both our attention mechanism and BERT ~\cite{devlin2018bert} are based on it.

